The Extended Parameter Filter

The parameters of temporal models, such as dynamic Bayesian networks, may be modelled in a Bayesian context as static or atemporal variables that influence transition probabilities at every time step. Particle filters fail for models that include such variables, while methods that use Gibbs sampling of parameter variables may incur a per-sample cost that grows linearly with the length of the observation sequence. Storvik devised a method for incremental computation of exact sufficient statistics that, for some cases, reduces the per-sample cost to a constant. In this paper, we demonstrate a connection between Storvik's filter and a Kalman filter in parameter space and establish more general conditions under which Storvik's filter works. Drawing on an analogy to the extended Kalman filter, we develop and analyze, both theoretically and experimentally, a Taylor approximation to the parameter posterior that allows Storvik's method to be applied to a broader class of models. Our experiments on both synthetic examples and real applications show improvement over existing methods.

==> separability.tex <==
In this section, we define a condition under which there
exist efficient updates to parameters. 
Again, we focus on the state-space model as described in
\figref{fig:graphmodel} and \eqref{eq:state-space-model}. The model in \eqref{eq:state-space-model} can also be expressed as
\beq
	x_t = f_{\theta}(x_{t-1}) + v_t \nn \\
	y_t = g_{\theta}(x_t) + w_t
\eeq
for some suitable $f_{\theta}$,$g_{\theta}$,$v_t$ and $w_t$.

\begin{defn}
A system is \emph{separable} if the transition function $f_{\theta}(x_{t-1})$ can be written as $f_{\theta}(x_{t-1})=g(x_{t-1})^Th(\theta)$ for some $f(\cdot)$ and $g(\cdot)$ and the stochastic i.i.d. noise $v_t$ has a log-polynomial density.
\end{defn}

\hide{
\begin{defn}
A transition model $p(x_t \given x_{t-1}, \theta)$ is \em{separable} if it can be written as $p(x_t \given x_{t-1}, \theta) =  g(x_t, x_{t-1})^T h(\theta, T(x_t, x_{t-1})) $, for some functions $g(\cdot)$, $h(\cdot)$ and $T(\cdot)$.
\end{defn}

\reminder{alternative definition}
\begin{defn}
A transition model $p(x_t \given x_{t-1}, \theta)$ is \em{separable} if it can be written as $p(x_t \given x_{t-1}, \theta) =  \exp( g(\theta) \cdot T(x_{t-1}, x_t) - A(\theta) + B(x_{t-1}, x_t) )$, for some functions $g(\cdot)$, $T(\cdot)$, $A(\cdot)$, and $B(\cdot)$.
\end{defn} }

The models defined in equation \ref{eq:storvik_model} is a subset of the model class which we define as \emph{separable}. The sufficient statistics exist for the static parameter if the states and the parameters are separable (this condition is sufficient but not necessary).
The class of Gaussian system processes is evidently separable in this sense, since the transition function  $\mymat{F}_k^T\beta=(\myvec{F}_k)^T\beta$, but the property applies to a much broader class of systems.
\begin{theorem}
\label{thm:separability}
For a separable system, there exists sufficient statistics for the Gibbs density, $p(\theta \mid x_{0:T},y_{0:T})$.
\end{theorem}

\hide{
\begin{theorem}
\label{thm:separability}
In state-space models defined in \eqref{eq:state-space-model}, if the transition function is {\em separable} and $\theta$ is only involved in transition, there exists sufficient statistics for the Gibbs density, $p(\theta \mid x_{0:T},y_{0:T})$.
\end{theorem} }
The proof is straightforward by Fisher-Neyman theorem\reminder{to cite??}, with and full details are given in appendix \ref{sec:appendix3}.

Therefore, Storvik's approach is easily applicable to separable models since there exists sufficient statistics that can be updated in constant time. Our algorithm will introduce a density approximation step which uses a polynomial approximation of either the Gibbs distribution $p(\theta \mid x_{0:t},y_{0:t})$ or the transition model. With this density approximation we will be imposing separability on a non-separable model in some approximate fashion.

